DEAR: A Novel Deep Learning-based Approach for Automated Program Repair

The existing deep learning (DL)-based automated program repair (APR) models are limited in fixing general software defects. % We present {\tool}, a DL-based approach that supports fixing for the general bugs that require dependent changes at once to one or multiple consecutive statements in one or multiple hunks of code. % We first design a novel fault localization (FL) technique for multi-hunk, multi-statement fixes that combines traditional spectrum-based (SB) FL with deep learning and data-flow analysis. It takes the buggy statements returned by the SBFL model, detects the buggy hunks to be fixed at once, and expands a buggy statement $s$ in a hunk to include other suspicious statements around $s$. We design a two-tier, tree-based LSTM model that incorporates cycle training and uses a divide-and-conquer strategy to learn proper code transformations for fixing multiple statements in the suitable fixing context consisting of surrounding subtrees. We conducted several experiments to evaluate {\tool} on three datasets: Defects4J (395 bugs), BigFix (+26k bugs), and CPatMiner (+44k bugs). On Defects4J dataset, {\tool} outperforms the baselines from 42\%--683\% in terms of the number of auto-fixed bugs with only the top-1 patches. On BigFix dataset, it fixes 31--145 more bugs than existing DL-based APR models with the top-1 patches. On CPatMiner dataset, among 667 fixed bugs, there are 169 (25.3\%) multi-hunk/multi-statement bugs. {\tool} fixes 71 and 164 more bugs, including 52 and 61 more multi-hunk/multi-statement bugs, than the state-of-the-art, DL-based APR models.

==> demo/fse21-demo-arch.tex <==
\section{System Architecture}
\label{sec:arch}

\begin{figure*}[t]
	\centering
	\includegraphics[width=5.4in]{fse21-demo-dear-arch.png}
%        \vspace{-0.12in}
        \caption{System Architecture}
        %\vspace{-0.06in}
	\label{fig:arch}
%         \vspace{-6pt}
\end{figure*}

Figure~\ref{fig:arch} shows {\tool}'s system architecture. The input
includes the buggy source code and the set of test cases. The output
is the ranked list of candidate patches.

\subsubsection*{\bf Fault Localization and Buggy-Hunk Detection}

(Section~\ref{sec:hunk-detection}). We first use a SBFL tool to locate
buggy statements with their suspiciousness scores. Our hunk detection
algorithm will use those statements to detect buggy hunks that need to
be fixed together.


\subsubsection*{\bf Multi-Statement Expansion}

(Section~\ref{sec:expansion}). Because SBFL might return only one
statement for a hunk, we have to expand to potentially include more
consecutive buggy statements. For this, we combine a
RNN~\cite{Cho-2014} to classify statements and data-flow analysis.

\subsubsection*{\bf Tree-based Code Repair}

(Section~\ref{sec:code-repair}). We first derive the AST subtrees for
the buggy statements. We apply the tree-based code repair module on
the buggy AST subtrees for those buggy statements. This module has the
trained context learning model and the trained tree transformation
model.
%For each buggy subtree~$T$, we summarize it and use the resulting AST
%as the input to the first trained LSTM model to produce the fixed AST
%with the summarized nodes. The fixed AST is encoded into a vector and
%combined with the vector for the buggy subtree $T$ into the input for
%the second trained LSTM model.
The result is the fixed subtrees corresponding to the candidate
patches. We apply grammatical rules and program analysis on the
current code to produce the fixed code. We perform re-ranking and
validate the fixed code using test cases as in DLFix~\cite{icse20} to
produce the final list of candidate results.



%\subsubsection{{\bf Training Process}}

%The input for training includes the source code before and after a
%fix (Figure~\ref{Fig:train}), which is parsed into ASTs. We then
%use CPatMiner~\cite{icse19-cpatminer} to compare them to derive the
%{\em changed, inserted}, and {\em removed} subtrees. As a result, the
%AST subtrees for the buggy statements are mapped to the respective
%fixed subtrees.

%{\bf 1. Fixing-Context Learning}~(Section~\ref{contextlearning:sec}).
%For each buggy subtree $T$ corresponding to a buggy statement, we need
%to build the fixing context and its corresponding context (step 1). To
%build the fixing context $C_b$ for $T$, we take the AST and collapse
%the structure of $T$ into a summarized node, and replace other buggy
%subtrees in the AST with the corresponding fixed subtrees. The
%corresponding (fixed) context $C_f$ of $T$ is similarly handled as
%$C_b$ with summarization, however, no such replacement is needed
%(because the code is fixed). The pair of $C_b$ and $C_f$ is used for
%training at the input layer and the output layer of a tree-based LSTM
%model~\cite{Tai-2015} (step 2). The vectors computed from this
%learning are used as additional weights (step 3) in code
%transformation learning next.

%{\bf 2. Code-Transformation Learning}~(Section~\ref{codetrans:sec}).
%To learn code transformations for fixing (step 4,
%Figure~\ref{Fig:train}), each buggy subtree $T$ itself and its fixed
%subtree $T'$ after the fix are used at the input layer and the output
%layer of another tree-based LSTM for training it.  Moreover, the
%fixing context computed as the vector in fixing-context learning is
%used an additional input in this step.







==> demo/fse21-demo-code-repair.tex <==
\section{Tree-based Code Repair}
\label{sec:code-repair}

\input{fse21-demo-training}

\input{fse21-demo-context-learning}

\input{fse21-demo-transformation-learning}

\input{fse21-demo-tree-repair}


==> demo/fse21-demo-context-learning.tex <==
\subsubsection{Training the Context Learning Model}
\label{sec:ctx-learning}

%\subsubsection{{\bf Building Fixing Context for Input Layer and Corresponding Context for Output Layer} (Figure~\ref{Fig:example_context})}
%\label{fixing-context}


For each pair of the buggy AST $I_1$ and the corresponding fixed AST
$O_1$, we perform alpha-renaming on the variables and consider each
statement node as a sentence and each code token as a word.  Next, we
use GloVe~\cite{glove2014} to produce the same tree structures of
$I_1$ and $O_1$ by replacing the AST nodes with their GloVe vectors.

For each of the buggy subtrees, we process as follows. For a buggy
subtree, we perform summarization and replacement. For summarization,
we use TreeCaps~\cite{treecaps} to produce the vector $V_s$ for the
tree structure rooted at the that buggy subtree. Moreover, for each of
the other buggy subtrees, we replace it with the corresponding fixed
subtrees. The idea is to have the model learn the correct surrounding
code context for a fix of a subtree. If we did not do the replacement,
the model will learn from the incorrect surrounding context for a fix.
The resulting tree after summarization and replacement is used at the
{\em input layer} of the tree-based LSTM model to learn the fixing
contexts. For the corresponding fixed subtree, we perform only the
summarization by using TreeCaps~\cite{treecaps} to produce the vector
$V'_s$ for that fixed subtree. The resulting tree after summarization
is used at the {\em output layer} of that tree-based LSTM model for
context learning. The summarization vectors $V_s$ and $V'_s$ will be
used as the weights to train the tree-based LSTM code transformation
model. We repeat the same process for all buggy subtrees in the buggy
AST.

%We then encode each AST node with the vector using the word embedding
%technique GloVe~\cite{glove2014}, which captures well overall
%structure.  We use those vectors to label the AST nodes in $I_1$ and
%$O_1$.  The resulting ASTs after this step are called the vectorized
%buggy AST $I_2$ and the vectorized fixed AST $O_2$
%(Figure~\ref{Fig:example_context}).
%
%Next, we perform differently for a buggy $S$-subtree $T_b$ and the
%corresponding fixed $S$-subtree $T_f$. For each buggy $S$-subtree in
%$I_2$, we perform {\em node summarization} and {\em replacement}. For
%node summarization, we use TreeCaps~\cite{treecaps} to capture sub-tree
%structure. For each of the other buggy $S$-subtrees, we replace it
%with the corresponding fixed $S$-subtree. In
%Figure~\ref{Fig:example_context}, the subtree [$V_3,V_4,V_5]$ is
%summarized into $V_b$, and the subtree [$V_7,V_6$] is replaced with
%[$V_7,V_4$] because \code{return b} was fixed into \code{return a}. The
%resulting AST, $I_3$, is used as the fixing context for
%the buggy $S$-subtree $T_b$ and used at {\em the input layer} of the
%encoder in the LSTM model.

\begin{figure}[t]
	\centering
	\includegraphics[width=3.4in]{fse21-demo-context-training.png}
	\vspace{-5pt}
	\caption{Fixing-Context Learning}
	\label{Fig:example_context}
%	\vspace{-10pt}
\end{figure}


%For each fixed $S$-subtree $T_f$ of $T_b$, we perform only node
%summarization since the fixed subtree provides the correct context. In
%Figure~\ref{Fig:example_context}, the fixed $S$-subtree
%[$V_3,V_4,V_6$] is summarized into $V_f$. The resulting AST, $O_3$
%after this task is used as the corresponding context for $T_f$ and
%used at {\em the output layer} of the decoder part in the LSTM
%model. Finally, the vectors $V_b$ and $V_f$ will also be used as the
%weighting input for the code transformation learning process.


==> demo/fse21-demo-expansion.tex <==
\section{Multi-Statement Expansion}
\label{sec:expansion}


%\input{sections/algorithm}

Because Ochiai does not aim to produce consecutive buggy statements in
a hunk, a detected buggy hunk from hunk detection algorithm might
contain only one statement. Therefore, we need to take the result
from Ochiai and expand each statement to potentially include more
consecutive statements in a hunk.

%A detected buggy hunk from the algorithm in
%Section~\ref{hunkdetect:sec} might contain only one statement because
%those statements are originally derived by
%Ochiai~\cite{abreu2006evaluation}, which does not focus on
%detecting~consecutive buggy statements in a hunk. Thus, we take the
%result from~Ochiai, and expand it to potentially include more statements
%in a hunk.

We use the seed buggy statement in a hunk and consider the surrounding
statements by first using a trained RNN~\cite{Cho-2014} model to
classify if the current statement under consideration is buggy or not.
The RNN model is trained as a classifier on the real buggy code. We
then use data-flow analysis to adjust the results because a
consecutive statement has a data dependency with a suspicious
statement is also suspicious.

%In general, to detect more buggy statements, we use
%RNN~\cite{Cho-2014} trained from real buggy code (explained later),
%and use data-flow analysis to adjust the results since a consecutive
%statement has a data dependency with a suspicious statement is also
%suspicious.

%The input of Multi-Statement Expansion algorithm
%(Algorithm~\ref{algo}) is the buggy statement \code{buggyS}, i.e.,
%the central statement of a given hunk. The output is a buggy hunk of
%consecutive statement(s).


%First, it produces a candidate list of buggy statements by including
%$N$ statements before and $N$ statements after \code{buggyS} ({\em
%  Expand2NCandidatesList} at line 2). In the current implementation,
%$N$=5.  Then, it uses a RNN model to act as a classifier to predict
%whether each buggy statement (except \code{buggyS}) in the candidate
%list is buggy or not ({\em RNNClassifier} at line 3). To train that
%RNN model, we use the real buggy statements in the buggy hunks in the
%training data (we will explain the model later).  We encode the
%statements using TreeCaps~\cite{treecaps} as in
%Section~\ref{fixing-context}.

%In {\em DataDepAnalysis} (line 4) to adjust the results from RNN, we
%first obtain {\em buggyHunk} surrounding the buggy statement
%\code{buggyS}, consisting of the statements before and after
%\code{buggyS}, that were predicted as buggy by the RNN model (line
%7).

We then examine statement-by-statement in the upward direction from
the center buggy statement in the buggy hunk
%candidate list of buggy statements
and in the downward direction as well. We will continue to expand
(upward or downward) in the current buggy hunk to include a statement
if it has a data dependency with the center buggy statement. We stop
the process (upward or downward), if we encounter a statement without
data dependency with the center statement or we exhaust the candidate
list in the buggy hunk. Finally, the buggy hunk containing consecutive
buggy statements is returned.

%\begin{figure}[t]
%	\centering
%	\includegraphics[width=3in]{graphs/expexample_2.png}
%        \vspace{-0.08in}
%	\caption{Multi-Statement Expansion}
%        \vspace{-0.06in}
%	\label{Fig:expansion}
%	\vspace{-15pt}
%\end{figure}



%Figure~\ref{Fig:expansion} shows an
%example. Ochiai~\cite{abreu2006evaluation} returns the buggy
%statement at line 4. First, the statements are encoded into vectors
%by TreeCaps. We expand from the statement at line 4 upward to include
%line 3 (even though RNN predicted it as non-buggy), since~it has a
%data dependency with the buggy statement at line 4 via the variable
%\code{c}. We also include line 5 because RNN predicts the statement
%at line 5 also as buggy.  At this time, we stop the upward and
%downward directions because we encounter the statements at line 2 and
%at line 6 that do not have data dependency with line 4.  The final
%result includes the buggy statements at lines 3--5 as the buggy hunk.



%\vspace{0.03in}

%\noindent {\bf \em \underline{Using RNN to predict if a statement is buggy.}} Let us explain how we use GRU-based RNN model~\cite{Cho-2014} to predict a buggy statement.

%\noindent {\bf 1. Training.} Input: all the buggy and non-buggy
%statements in all the hunks in the training dataset. We directly use
%the neural architecture of the GRU-based RNN model in~\cite{Cho-2014}.
%We use TreeCaps~\cite{treecaps} to encode each statement with a
%vector to capture its structure.

%The RNN model operates in the time steps. At the time step $k$
%($k$>=1), at the input layer, GRU consumes the TreeCaps vector of
%the $k^{th}$ statement $S_k$. At the output layer, $S_k$ is labeled as
%1 if it is a buggy statement and as 0 otherwise. Moreover, in addition
%to the input at the time step $k+1$, we also feed the output of the
%time step $k$ to the GRU.

%\noindent {\bf 2. Prediction.} The trained GRU-based RNN model is used
%in Algorithm~\ref{algo} at line 3 to predict if a statement in the
%hunk is considered buggy or not. It takes a statement in the form of a
%TreeCaps vector. The model takes the vectors of all the statements in
%a hunk and labels them as buggy or non-buggy in multiple time
%step manner.


==> demo/fse21-demo-hunk-detection.tex <==
\section{Fault Localization and Hunk Detection}
\label{sec:hunk-detection}

Given the source code under study and the set of test cases, our
algorithm first uses Ochiai~\cite{abreu2006evaluation} to produce a
ranked list of buggy statements with the associated suspiciousness
scores. From this list, our algorithm aims to compute the buggy
hunk(s) that need to be fixed together at once in the same patch.

To achieve that goal, we use the pre-trained BERT
model~\cite{devlin2018bert}.~We first learn the {\em fixing-together
  relationships among the statements}, and then derive the
fixing-together relationships among the buggy~hunks.

%To fix multi-hunk, multi-statement bugs, our extended FL needs to {\em
%  detect buggy hunk(s) that are fixed together in the same patch}. To
%this end, we directly fine-tune Google's pre-trained BERT
%model~\cite{devlin2018bert} to learn the {\em fixing-together
%  relationships among statements first}, and then derive such
%relationships among buggy hunks.

Let us explain how we fine-tune BERT and use it to derive
fixing-together buggy hunks.

\subsubsection*{Fine-tuning BERT}
Let $H$ be a set of the hunks that are fixed together for a bug. The
input for the training process is all the sets $H$s for all the bugs
in the training set.

\underline{Step 1}. For a pair of hunks $H_i$ and $H_j$ in $H$, we
take every pair of statements $S_k$ and $S_l$, one from each hunk, and
build the vectors with BERT. We consider the pair of statements
($S_k$, $S_l$) as being ``fixed-together''.

\underline{Step 2}. Step 1 is repeated for all the pairs of the
statements ($S_k$, $S_l$)s in all the pairs $H_i$ and $H_j$ in $H$.
We also repeat Step 1 for all $H$s. We use them to fine-tune the BERT
model to learn the fixing-together relationships among two
statements in two hunks.

%We repeat step 1 for all such the pairs ($S_k$, $S_l$)s in $H$ and for
%all $H$s, and use them to train/fine-tune the BERT model to learn
%fixing-together relationships among two statements in two hunks.

\subsubsection*{Using Fine-tuned BERT for Hunk Detection} The input of
of this procedure is the fine-tuned BERT model and buggy code $P$.
The output is the groups of hunks that need to be fixed together.

\underline{Step 1}. Ochiai~\cite{abreu2006evaluation} is run on the
source code and the test cases. It returns the list of buggy
statements and suspiciousness scores.

\underline{Step 2}. The consecutive statements within a method
returned by Ochiai are grouped together to form the hunks $H_1$,
$H_2$, ..., $H_m$.

\underline{Step 3}. To decide if a pair of hunks ($H_i$,$H_j$) needs
to be fixed together, we use the BERT model that was
fine-tuned. Specifically, for every pair of statements ($S_k$,$S_l$),
one from each hunk ($H_i$,$H_j$), we use the fine-tuned BERT model to
measure the fixing-together relationship score for ($S_k$,$S_l$). The
fixing-together score between $H_i$ and $H_j$ is the average of
the scores of all the statement pairs within each of those two hunks.
%If the average score for all the statement pairs is higher than a
%threshold, we consider ($H_i$,$H_j$) as needed to be fixed
%together.
From the pairs of detected hunks, we build the groups of
fixing-together hunks.


==> demo/fse21-demo-intro.tex <==
\section{Introduction}
\label{sec:intro}

{\em Automated Program Repair} (APR) approach is aimed to help
developers in automatically identifying and fixing the defects in
their programs. There have been several APR approaches that can be
classified into three groups: 1) search-based APR, 2) software
mining-based APR, and 3) machine learning (ML)-based APR (including
deep learning (DL) approaches). First, the search-based APR
approaches~\cite{LeGoues-icse12,le2011genprog,martinez2016astor,qi2014strength}
aim to search for the repairs by performing the mutations on the buggy
code in the solution space. Second, the software mining-based APR
approaches\cite{kim2013automatic,le2016history,liu2019avatar,tbar-issta19,nguyen2013semfix,icse10,ray-fse12}
mine and learn the fixing patterns from the prior fixes in the same or
different projects. Third, several approaches leverage ML to
implicitly learn fixing patterns from the training
data~\cite{long2016automatic,long2017automatic,saha2017elixir}.  Deep
Learning (DL)-based APR approaches have treated the bug-fixing problem
as machine translation from buggy code to the fixed
one~\cite{chakrabortycodit,chen2018sequencer,hata2018learning,tufano2018empirical,see2017get,tufano2019learning,icse20}. Other
DL-based approaches learn similar fixes for similar
bugs~\cite{gupta2017deepfix,white2019sorting,white2016deep}.

%Researchers have proposed several approaches to help developers in
%automatically identifying and fixing the defects in programs. Such
%approaches are referred to as {\em automated program~repair}
%(APR). The APR approaches have been leveraging various techniques in
%the areas of {\em search-based software engineering}, {\em software
%  mining}, {\em machine learning (ML)}, and {\em deep learning (DL)}.

%For {\em search-based
%  approaches}~\cite{LeGoues-icse12,le2011genprog,martinez2016astor,qi2014strength},
%a search strategy is performed in the space of potential solutions
%produced by mutating the buggy code via operators. Other approaches use
%software mining to {\em mine and learn fixing patterns} from prior bug
%fixes \cite{kim2013automatic,le2016history,liu2019avatar,tbar-issta19,nguyen2013semfix}
%or cloned code~\cite{icse10,ray-fse12}. Fixing patterns are at the
%source code level \cite{liu2019avatar,tbar-issta19} or at the change
%level~\cite{wen2018context,Simfix,koyuncu2018fixminer}.  {\em Machine
%  learning} has been used to mine fixing patterns and the candidate
%fixes are ranked according to their
%likelihoods~\cite{long2016automatic,long2017automatic,saha2017elixir}.
%While some DL-based APR approaches learn similar
%fixes~\cite{gupta2017deepfix,white2019sorting,white2016deep}, other
%ones use machine translation or neural network models with
%various~code~abstractions to generate
%patches~\cite{chakrabortycodit,chen2018sequencer,hata2018learning,tufano2018empirical,see2017get,tufano2019learning,icse20}.

Despite the benefit of implicitly learning fixing patterns, the
existing DL-based APR approaches still do not support well the fixes
that {\em involve dependent changes to multiple statements in one or
  multiple hunks of code at once}. Currently, the state-of-the-art
DL-based APR approaches fix one statement at a time. Thus, it can only
fix the bugs with independent changes. However, if one uses such a
individual-statement DL-based APR tool to fix a bug that requires
dependent changes by modifying one statement at a time, the tool
treats that statement as incorrect and all other statements as
correct. This is not true because during fixing the current statement,
the remaining statements might not be fixed to correct code yet. In
other words, it does not work if one uses an individual-statement
DL-based APR tool to fix the multi-hunk/multi-statement bugs that
require dependent changes to multiple statement at once.

%Despite their successes, the state-of-the-art DL-based APR approaches
%  are still limited in fixing the software defects that involve the
%  {\em fixing changes to multiple statements in the same or different
%  parts of a file or different files} (which are referred to as {\em
%  hunks}).  None of existing DL-based approaches can automatically
%  fix the bug(s) with {\em dependent changes to multiple statements
%  in multiple hunks at once}.
%The reason is that~if~we use an individual-statement DL-based APR tool
%on the current statement, the tool treats that statement as
%incorrect and treats the other statements as correct. This does not hold
%since during fixing the current statement, the remaining statements
%might not be fixed to correct code yet. Thus, it might be~inaccurate
%when using existing DL-based APR tools to fix individual statements
%for multi-hunk/multi-statement bugs.
%
%While DL provides benefits for fix learning, {\em this limitation
%  makes the~DL-based APR approaches less capable than the other
%  directions (search-based and pattern-based APR), which support
%  multiple-statement fixes.}

We propose {\tool}, a DL-based APR tool that supports fixing
for the bugs with {\em dependent changes at once to one or multiple
  buggy hunks, in which a hunk contains one or multiple buggy
  statements}.

%In this paper, we aim to advance deep learning-based APR
%by~introducing {\tool}, a DL-based model that supports auto-fixing for
%the bugs with {\em dependent changes at once to one or multiple buggy
%  hunks, in which a hunk contains one or multiple buggy
%statements}. To do that, we make three following key technical
%contributions.

To identify all the hunks of code that need to be fixed together, we
develop a {\em novel fault localization (FL) technique that combines
  traditional spectrum-based FL (SBFL) with machine learning and
  data-flow analysis}. We use Ochiai~\cite{abreu2006evaluation} to
produce a ranked list of suspicious statements and then compute the
buggy hunks that need to be fixed together by fine-tuning a
pre-trained BERT model~\cite{devlin2018bert}, which is trained on the
dataset of the bugs that were fixed at multiple statements in multiple
hunks. We also develop a {\em statement expansion algorithm} whose
goal is to take a statement in a hunk as a seed and expand it to
include more consecutive statements if needed. Our statement expansion
algorithm leverages a RNN model to detect if a statement is buggy and
uses data-flow analysis to make adjustment to the result to form a
buggy hunk.

After identifying the buggy hunks containing buggy statements, {\tool}
performs the fixes by tree-based code transformation. {\em To learn the
code transformation for fixing, we enhance a two-layer, tree-based
LSTM model in DLFix~\cite{icse20}}. In the first layer, the model is
trained to learn the fixing context, i.e., the AST structures
surrounding a buggy AST subtree. The fixing context represented by a
vector will be used as a weight in the learning at the second layer,
which learns the code transformation from a buggy AST subtree to the
fixed one. To train that LSTM model, we use a divide-and-conquer
strategy to more accurately learn fine-grained code structure
transformations of a fix. To do so, we use an AST-based differencing
technique to derive the fine-grained, AST-based changes for the
mapping between each pair of buggy and fixed code in the training
dataset. Those fine-grained mappings help the LSTM model avoid
incorrect alignments of buggy and fixed code.

The screenshots, source code, and data are available in our
website~\cite{autofix-website} and Github
repository~\cite{AutoFix2021}.

%First, we develop a {\em fault localization (FL) technique for
%  multi-hunk, multi-statement patches that combines traditional
%  spectrum-based FL (SBFL) with DL and data-flow analysis}. {\tool}
%uses a SBFL method to identify the ranked list of suspicious buggy
%statements. Then, it uses that list of buggy statements to {\em derive
%  the buggy~hunks that need to be fixed together} by fine-tuning the
%pre-trained BERT model~\cite{devlin2018bert}, to learn the
%fixing-together relationships among statements. We also design an
%expansion algorithm that takes a buggy statement $s$ in a hunk as a
%seed, and expands to include other suspicious consecutive statements
%from $s$. To achieve that, we use an RNN model to classify the
%statements as buggy or not, and use data flow analysis for adjustment
%and then form the hunks.

%Second, after the expansion step, we have identified all the buggy
%hunk(s) with buggy statement(s). We develop a {\em compositional approach
%to learning and then generating multi-hunk, multi-statement
%fixes}. Toward that end, from the buggy statements, we derive the
%corresponding subtrees of Abstract Syntax Tree (AST). For each buggy
%subtree, we encode it as a vector representation and apply a
%tree-based Long Short-Term Memory (LSTM) model to derive the fixed
%code. To train that LSTM model, we use a divide-and-conquer strategy
%to more accurately learn fine-grained code structure transformations
%of a fix. To do so, we use an AST-based differencing technique to
%derive the fine-grained, AST-based changes for the mapping between each pair
%of buggy and fixed code in the training dataset. Those fine-grained
%mappings help the LSTM model avoid incorrect alignments of buggy and
%fixed code.

%Third, we have enhanced a two-layer, tree-based LSTM model in
%DLFix~\cite{icse20} with {\em an attention layer and a cycle training}
%to help {\tool} to learn the proper code fixing changes in the
%suitable context of surrounding code. In the first layer, it learns
%the fixing context,~i.e., the code structures surrounding a buggy AST
%subtree. In the second layer, it learns the code transformations to
%fix that buggy subtree using the context as an additional
%weight. Finally, in training,~to learn better the fixing context
%for a buggy subtree, we use the subtrees {\em after the fix} for
%the other buggy subtrees to train {\tool}, instead of using those
%buggy ones (in training, the fixed subtrees for all buggy ones are
%known). That is, it is better to train the model to learn the context
%for a buggy subtree from the fixed surrounding code
%(i.e., subtrees after the fix), rather than the un-fixed subtrees.


==> demo/fse21-demo-new-ideas.tex <==
\section{Novel Aspects in {\tool}}
\label{sec:new-ideas}

In comparison with the state-of-the-art, ML-based APR approaches, we
have the following novelties in {\tool}.

\subsubsection*{\bf 1. A Novel Fault Localization Technique for
  Multi-hunk, Multi-Statement Patches} Due to the need of supporting
fixes involving multiple hunks with multiple statements, we develop
our fault localization technique in Section~\ref{sec:hunk-detection}.
This technique extends Ochiai~\cite{abreu2006evaluation}, a
spectrum-based FL with machine learning as well as the data-flow
analysis. The two novel components in our FL technique include:


1) {\bf \em Hunk-Detection Algorithm}: we use DL to detect the hunks
of code that need {\em to be changed together in the same patch},
because SBFL tool returns the suspicious candidates for the fault, but
not necessarily needed to be fixed together.

2) {\bf \em Statement Expansion Algorithm}: the algorithm takes each
of those detected fixing-together hunks and expands it to include
potential consecutive suspicious statements in the hunk.

%Our approach combines traditional spectrum-based FL (SBFL) with DL and
%data-flow analysis. Specifically, we use a SBFL technique to obtain a
%ranked list of candidate statements to be fixed with their
%suspiciousness scores. We need to extend the result from SBFL in two
%tasks. First, we design a {\bf \em hunk-detection algorithm} to use DL
%to detect the hunks of code that need {\em to be changed together in
%  the same patch}, because SBFL tool returns the suspicious candidates
%for the fault, but not necessarily needed to be fixed
%together. Second, we design {\bf \em an expansion algorithm} that
%takes each of those detected fixing-together hunks and expands it
%to include other consecutive suspicious statements in the hunk.

%A fault localization (FL) tool returns a ranked list of candidate
%statements that need to be fixed together with suspiciousness
%scores. We develop an algorithm taking a suspicious statement returned
%from a FL tool, then detecting the buggy hunks and expanding to
%include other suspicious ones using a~combination of machine learning
%and program analysis.


%In Figure~\ref{fig:motiv}, the SBFL tool returns line 5
%as a suspicious one. After hunk detection, {\tool} uses data
%dependencies via the variable \code{retrieve$\_$password} to include
%the statement at line 10 as to be fixed.




%Firstly, in order to fix the multiple statements bugs, after getting the results from fault localization, we need to have the expansion step to expand the located buggy lines in order to find correct fixing positions. Having a expansion step to get the correct statement location is one of the most important different points comparing with state-of-art automated program repairing approaches. For example, in figure \ref{fig:motiv}, the fault localization can only let us know that the \textit{line 5} is buggy, but the \textit{line 10} cannot be located as buggy. By using the expansion step, because \textit{line 5} and \textit{line 10} have the similar variable \textit{retrieved\_password}, \textit{line 10} will be expanded as a buggy which can help our model to do the repairing in the right statements.


%\vspace{0.03in} \noindent {\bf 2. [Divide-and-Conquer Strategy with
%    Fine-grained, AST change detection]}:

\subsubsection*{\bf 2. A Compositional Approach to
  Learning and Generating multi-hunk, multi-statement fixes} Because
we have to learn and generate the fixes involving multiple hunks with
multiple statements, we use a compositional approach with a {\em
  divide-and-conquer} strategy. When learning, we treat each buggy
subtree and use the fixed code for other buggy subtrees to form
the context for the fix to that buggy subtree. When fixing, we make
the tree-based code transformations for all buggy trees at once
as explained in Figure~\ref{Fig:repair}.

For fixing involving multiple statements, a naive approach would let
the DL model learn the code structure changes and make the alignment
between the code structures before and after the fix. With the
$m$-to-$n$ statement changes, a model might incorrectly align the
statements. To facilitate code transformation learning, during
training, we leverage a fine-grained AST-based change detection to map
the ASTs before and after the fix. Such mappings enable {\tool} to
learn the fixing changes at more {\em localized structures}.

%To auto-fix a bug with multiple statements, a tool needs to make
%$m$-to-$n$ statement changes, i.e., $m$ statements might generally
%become $n$ statements after the fix. A naive approach would let a
%model learn the code structure changes and make the alignment between
%the code before and after the fix. Because a fix involves structural
%changes as in Observation 2, during training, a model might
%incorrectly align the code before and after the fix, thus, leading to
%incorrect learning of the fixes. For example, without this step, the
%model might map \code{retrieved\_password} at line 10 to the same
%variable at line 6 (correct map is line 11).
%
%Thus, to facilitate the code transformation learning for bug fixing,
%during training, we use {\em a divide-and-conquer strategy via
%  fine-grained, AST change detection}.
%
%We integrate into {\tool} a fine-grained AST-based change detection to
%map the ASTs before and after the fix. Such mappings enable {\tool} to
%learn the fixing changes at more {\em localized structures}.
%
%That is, during training, we use {\em a divide-and-conquer strategy
%  with fine-grained, AST change detection}.
%
%For example, after using fine-grained AST change detection, we know
%that the statements at lines 4--5, and 7 become the statements at
%lines 4, and 6--9; and the statement at line 10 becomes the one at
%line 11. We can break them into two groups and align the corresponding
%statements for the model to~learn.

%so that the model can avoid incorrect alignments and learn the code
%transformations more accurately.

%Secondly, in multiple statements situation, it is hard to know what the code structure should be like after fixing. To improve this point, we would like to use part of the technique from existing study \cite{}. In this study, it can do the node changing mapping in AST. We would like to this part in our approach and we call it code structure change mapping. We could map the statements before fixing and after fixing by knowing the node changes mapping. In this way, we can know how the statement could be changed to decrease the difficulty of automated program repairing. For example, in figure \ref{fig:motiv}, with the code structure change mapping, we could know the \textit{line 5} could be fixed into \textit{line 4, line 6-9} and \textit{line 10} could be fixed into \textit{line 11}. In this way, the complex multiple statement fixing could be a one statement to three statements fixing and a one statement to one statement fixing. It is much easier for the model to learn and fix. And also, it can avoid the model mapping the statement to wrong position. For example, without this point, the model may map the \textit{line 10} with \textit{line 6}. Because they both have the variable \textit{retrieved\_password}.

\subsubsection*{\bf 3. Fixing Multiple Subtrees at once}

%We deal with the fixes having multiple statements in one or multiple
%hunks by modifying the design and orchestration of the DLFix
%model~\cite{icse20} with the use of attention layer and cycle training
%(Section~\ref{contextlearning:sec}).

While DLFix fixes one subtree at a time, we modify it to fix multiple
subtrees at once. In the first layer, we {\em collapse the structural
  changes to multiple subtrees of a fix into multiple summarized
  nodes} as seen in Figure~\ref{Fig:example_context}. This strategy
allows the model to learn the code transformation w.r.t. a fix
in the right context of surrounding code.
%to learn the fixing context.
%
In the second layer, for each summarized node, {\tool} learns the code
transformations corresponding to the structural changes of a subtree
before and after the fix using the fixing context learned from the
first layer.
%$as an emphasis weight. This enables learning the fixes
%specific to a surrounding context.

%For example, during training, after marking the AST subtrees of the
%statements at line 5 and line 10 before the fix as buggy,~{\tool} {\em
%  replaces} them with the two ``summarized'' nodes and then learns the
%fixing context consisting of the surrounding nodes in the method.~We
%``summarize'' the subtrees with vector representations
%(Section~\ref{fixing-context}). In the second layer, as in DLFix,
%{\tool} learns the transformations from the subtree for the
%statement at line 5 into the subtree for the fixed statements at the
%lines 6, 7--9, and learns the transformations from the subtree for the statement at line 10 to the one at line 11.

\subsubsection*{\bf 4. Transformation Learning with
  Correct Surrounding Code Context} In training, to learn the fix for
a subtree if there are multiple buggy subtrees, we need to make sure
that the context of surrounding code for the model to learn is
correct.  Thus, we need to feed into the model {\em the other
  surrounding statements} {\em after the fix} (see the ``Replace''
arrow in Figure~\ref{Fig:example_context}).
%For example, for training, to learn the fix to the statement at line
%5 with \code{toUpperCase}, a model needs to integrate the fixed
%version of the other buggy line, i.e., the code at line 11 with
%\code{passwordHash} as the fixing context (instead of the buggy code
%at line 10).
If the surrounding code before the fix is used, the model will learn
the incorrect context for fixing the current buggy subtree.


==> demo/fse21-demo-post-processing.tex <==
\subsection{Post Processing}
\label{sec:post}

We use a similar post-processing procedure as in DLFix~\cite{icse20}.
%A naive approach would face combinatorial explosion in forming the
%candidate fix(es) because for each node in the sub-tree, we maintain
%top-5 candidates. However,
When we combine the candidates for all the nodes in the fixed
sub-tree, we apply several filters to verify the syntaxes and
semantics of the candidates as in DLFix~\cite{icse20}.
Many invalid candidates in the current method in the
project are filtered.
%Therefore, when we form a candidate by combining all the candidates
%for the nodes, we apply a set of filters to verify the program
%semantics in the same manner as in DLFix~\cite{icse20}. This allows us
%to eliminate invalid candidates immediately.
We use the alpha-renaming filter to change the names back to the
normal Java code with the right types, the syntax-checking filter to
remove the candidates with syntax errors, and the name validation
filter to check the validity of the variables, methods, and classes.
%Moreover, for further improvement, we use beam search in
%maintaining only the top-ranked candidate fixes. Thus, we do not
%exhaust all compositions in forming the statements. This helps
%maintain a manageable number of candidates.
We also use re-ranking to improve the ranking of the candidate
patches.
%After going through all the filters, we also used the re-ranking
%scheme as in DLFix~\cite{icse20} to re-rank the candidate patches.
%
%After passing the above filters, we used the CNN-based ranker in
%\cite{icse20} to re-rank the candidate patches.  Particularly, the
%ranker uses GloVe~\cite{glove2014} to learn vectors for each character
%in each candidate patch.  The ranker views each candidate patch as a
%sequence of character vectors and takes all patches as the input for a
%CNN model with a softmax function to do the re-ranking based on the
%classification scores.  We trained the ranker with previous fixes in
%our dataset.
Finally, we use test cases for patch validation. We test all the
candidate patches.

%With the re-ranked candidate patches, we used test cases to conduct
%patch validation. We verify each patch from the top to the bottom
%until a correct patch is identified and the patch validation ends.
%If all candidate patches for fixing a location cannot pass all the
%test cases, we select the next location to repeat the process.


==> demo/fse21-demo-related.tex <==
\section{Related Work}

\noindent{\bf Deep Learning-based APR approaches}. 
%Deep learning (DL) has been applied in APR.  
%The first group of DL-based APR approaches leverage the capability of DL models in {\em learning similar source code for similar fixes}.  
%Some DL APR tools learn similar code for similar fixes. For example, 
DeepRepair~\cite{white2016deep} learns code similarities to select the repair ingredients
from code fragments similar to the buggy code.
DeepFix~\cite{gupta2017deepfix} learns the syntax rules to fix syntax errors.
%uses deep learning to directly generate patches. The precision of this approach depends on the neutral network learned from the training
%set. However, so far this approach is only evaluated
%on syntactic errors.
%Some other approaches treat APR as a {\em statistical machine translation} that translates the buggy code to the fixed code. 
Some other approaches use translation models to directly translates the buggy code to the fixed code. 
Ratchet~\cite{hata2018learning}, Tufano {\em et
	al.}~\cite{tufano2018empirical}, and SequenceR~\cite{chen2018sequencer} mainly use neural network machine translation (NMT) with
attention-based Encoder-Decoder and code abstractions to
generate patches. 
%sequence-to-sequence NMT with a copy mechanism~\cite{see2017get}.
CODIT~\cite{chakrabortycodit} encodes code structures, learns code edits, and adopt an NMT model to suggest fixes. 
%The comparison with these NMT-based APR approaches is provided in the introduction. 
Tufano {\em et al.}~\cite{tufano2019learning} learns code changes
using a sequence-to-sequence NMT with code abstractions and
keyword replacing. DLFix~\cite{icse20} has a tree-based
translation model to learn the fixes.
%It does not work for multi-statement bugs.
%
%It does not have multi-statement summarization, divide-and-conquer
%strategy, and expansion algorithm (it works only for single-statement
%fixes).
%In general, the above mentioned DL approaches normally can only fix
%one statement bugs.
The existing DL-based APRs fix individual statements at a
time, thus, cannot work well for multi-hunk/multi-stmt bugs.

%the bugs with dependent fixes to multiple statements.

%DLFix has been tested and can auto-fix more bugs than
%Ratchet~\cite{hata2018learning}, Tufano {\em et
%  al.}~\cite{tufano2018empirical}, CODIT~\cite{chakrabortycodit}, and
%Tufano {\em et al.}~\cite{tufano2019learning} on Defects4J and BigFix.
%In this paper, our empirical results show that \tool can auto-fix more
%bugs than DLFix and SequenceR.

\iffalse
%Let us discuss the related work on automated program repair (APR). In
%the earlier stage, the APR approaches aimed to automatically derive
%{\em the fixes for similar code} cloned from one place to
%another~\cite{icse10}, or similar code due to porting or
branching~\cite{ray-fse12}.  Ray and Kim~\cite{ray-fse12}
automatically detect similar fixes for similar code that are ported or
branched out. The code in different branches is almost similar,
thus, the fix can be reused.
%
FixWizard~\cite{icse10} automatically derives {\em the
	fixes for similar code} that were cloned from one place to another.
It can also work for the {\em code peers}, which are the code having similar
internal and external usages.

A large group of APR approaches has explored {\em search-based
	software engineering} to tackle more general types of
bugs~\cite{le2011genprog,qi2014strength,LeGoues-icse12,martinez2016astor}.
A search strategy is performed in the space of potential solutions
produced by several operators that mutate the buggy code. Then, the
test cases and/or program verification are applied to select the
better candidate fixes~\cite{smith2015cure}.
%
GenProg~\cite{le2011genprog} uses genetic search on repair mutations
and works at the statement level by inserting, removing or replacing a
statement taken from other parts of the same
program. RSRepair~\cite{qi2014strength} fixes buggy programs with
random search to guide the patch generation
process. MutRepair~\cite{martinez2016astor} attempts to generate
patches by applying mutation operators on suspicious if-condition
statements. Smith {\em et al.}~\cite{smith2015cure} showed that these
approaches tend to overfit on test cases, by generating incorrect
patches that pass the test cases, mostly by deleting functionalities.

PAR~\cite{kim2013automatic} is an APR approach that is based on fixing
templates that were manually extracted from 60,000 human-written
patches. Later studies (e.g., Le {\em et al.}~\cite{le2016history})
have shown that the six templates used by PAR could fix only a few
bugs in Defects4J. Anti-patterns were integrated in existing
search-based APR tools~\cite{tan2016anti} (namely,
GenProg~\cite{le2011genprog} and SPR~\cite{long2015staged}) to help
alleviate the problem of incorrect or incomplete fixes. A key
limitation of those search-based approaches is that they rely much on
the quality of mutation operations and the fixing patterns.
\fi

%\textbf{Hard-coded Rules based APR.}  Some existing APR techniques are
%mostly based on hard-coded rules and operators, defined by human
%experts, used to generate potential patches obtained with mutation
%operators for a buggy code.  For example, GenProg~\cite{le2011genprog}
%uses genetic search on repair mutations and works at statement-level
%by inserting, removing or replacing a statement taken from other parts
%of the same program.  RSRepair~\cite{qi2014strength} tries to fix
%buggy programs with the same mutation operations in GenProg but uses
%random search to guide the patch generation process.
%MutRepair~\cite{martinez2016astor} attempts to generate patches by
%applying mutation operators on suspicious if-condition statements.
%These approaches have several limitations, rooted in the fact that
%they are based on handcrafted rules with limited scope (i.e., single
%statements, limited number of mutation operators, specific parts of
%expressions).  Moreover, Smith et al.~\cite{smith2015cure} showed that
%these approaches tend to overfit on test cases, by generating
%incorrect patches that pass the test cases, mostly by deleting
%functionalities.

%Kim et al.~\cite{kim2013automatic} initiated with PAR a milestone of APR based on fix templates that were manually extracted from 60,000 human-written patches. Later studies (e.g., \cite{le2016history}) have shown that the six templates used by PAR could fix only a few bugs in Defects4J.
%~\cite{tan2016anti} manually define a set of patterns for patch generating or filtering based on repair history.
%Anti-pattern~\cite{tan2016anti} integrated anti-patterns into two existing
%search-based automated program repair tools (namely, GenProg~\cite{le2011genprog} and SPR~\cite{long2015staged}) to help alleviate the problem of incorrect or incomplete fixes resulting from program repair.
%In their study, the anti-patterns are defined by themselves and limited
%to the control flow graph. Additionally, their anti-patterns are
%not meant to solve the problem of deriving better patches
%automatically, provide more precise repair hints to developers.

\noindent{\bf Pattern-based APR approaches.}
%In contrast to the search-based approaches, 
%Some approaches 
Those approaches have {\em mined and learned fix patterns}
from prior fixes
\cite{nguyen2013semfix,le2016history,liu2019avatar,kim2013automatic},
either automatically or
semi-automatically~\cite{le2016history,nguyen2013semfix,liu2019avatar,tbar-issta19}.
%The mining process of the fix patterns/templates can be automatically
%or semi-automatically~\cite{le2016history,nguyen2013semfix,liu2019avatar,tbar-issta19}.
%SemFix~\cite{nguyen2013semfix} instead uses symbolic execution and constraint solving to synthesize a patch by replacing only the right-hand side of assignments or branch predicates.  
%Long and Rinard proposed 
Prophet~\cite{long2016automatic} learns code correctness models from a
set of successful human patches.  Droix~\cite{tan2018repairing} learns
common root-causes for crashes using a search-based repair.
%Prophet learns a patch ranking model using machine learning algorithm based on existing patches.  
Genesis~\cite{long2017automatic} automatically infers patch
generation from users' submitted
patches. HDRepair~\cite{le2016history} mines closed frequent bug fix
patterns with graph representations. ELIXIR~\cite{saha2017elixir} uses
templates from PAR with local variables, fields, or constants, to
construct expressive
repair-expressions. CapGen~\cite{wen2018context},
SimFix~\cite{Simfix}, FixMiner~\cite{koyuncu2018fixminer} rely on
frequent code changes extracted from existing
patches. Avatar~\cite{liu2019avatar} exploits fix patterns of static
analysis violations for patch generation.
%Tbar~\cite{tbar-issta19} collects all fix patterns from
%the existing APRs and investigates to what extent fix
%patterns are effective. Then,
Tbar~\cite{tbar-issta19} is a template-based APR tool with the
collected fix patterns.
Angelix~\cite{mechtaev2016angelix} catches semantic information to
repair methods.
%that scales up to programs of similar size as are handled by search-based repair tools.
ARJA~\cite{yuan2018arja} generates lower-granularity patch
representation enabling efficient searching.


%We compared {\tool} with Hercules~\cite{hercules-icse19} in Section V.
%The most recent and similar work to ours is Hercules~\cite{hercules-icse19} that can auto-fix multi-hunk bugs. However, we analyzed the fixed bugs (bug ids available in Hercules's paper) from Hercules and found that Hercules can only fix the hunks requiring one statement fixing. 

%Compared with the above tools, {\tool} is practical and general to work on all bug types without any assumption on bug types.
%, which allows us to make no assumptions before analyzing and fixing a program.

%Furthermore, {\tool} can auto-fix more bugs than any tool in the literature. 


%\textbf{Fix Pattern Mining and Learning based APR.}  Another direction
%of APR approaches tend to automatically mine fix patterns or
%templates.  For example, SemFix~\cite{nguyen2013semfix} instead uses
%symbolic execution and constraint solving to synthesize a patch by
%replacing only the right-hand side of assignments or branch
%predicates.  Long and Rinard also proposed a patch generation system,
%Prophet~\cite{long2016automatic}, that learns code correctness models
%from a set of successful human patches. Prophet learns a patch ranking
%model using machine learning algorithm based on existing patches.
%They further proposed a new system, Genesis~\cite{long2017automatic},
%which can automatically infer patch generation transforms from
%developer submitted patches for automated program repair.  Motivated
%by PAR~\cite{kim2013automatic}, more effective automated program
%repair systems have been explored. HDRepair~\cite{le2016history} was
%proposed to repair bugs by mining closed frequent bug fix patterns
%from graph-based representations of real bug fixes.  Nevertheless, its
%fix patterns, except the fix templates from PAR, still limits the code
%change actions at abstract syntax tree (AST) node level, but are not
%specific for some types of bugs.  ELIXIR~\cite{saha2017elixir}
%aggressively uses method call related templates from PAR with local
%variables, fields, or constants, to construct more expressive
%repair-expressions that go into synthesizing patches.  More recently,
%CapGen~\cite{wen2018context}, SimFix~\cite{jiang2018shaping},
%FixMiner~\cite{koyuncu2018fixminer} are further proposed to fix bugs
%automatically based on the frequently occurred code change operations
%(e.g., Insert If- Statement) that are extracted from the patches in
%developer change histories.  Avatar~\cite{liu2019avatar} exploits fix
%patterns of static analysis violations as ingredients for patch
%generation So far however, pattern-based APR approaches focus on
%leveraging patches that developer applied to semantic bugs.







%Despite of treating the APR as code transformation learning problem, their approach takes entire method as the context for a bug. Thus, it has too much noise, leading to lower effectiveness than {\tool}. In other words, the treatment of context from {\tool} helps improve over their model.


%DeepRepair~\cite{white2019sorting} is an early attempt to integrate machine learning in a program repair loop. DeepRepair leverages learned code similarities, captured with recursive autoencoders~\cite{white2016deep}, to select repair ingredients from code fragments that are similar to the buggy code.

%SequenceR~\cite{chen2018sequencer} is another Neural Machine Translation (NMT)-based system to learn source code changes based on a seq2seq model and copy mechanism~\cite{see2017get}. DeepRepair uses machine learning to select interesting code, SEQUENCER uses machine
%learning to generate the actual patch. However, as reported by SequenceR, it can only find 14 correct patches. Another approach using NMT, CODIT~\cite{chakrabortycodit}, has been proposed to learn code edits and recommend possible edits. However, CODIT uses tree-based NMT. Although CODIT is not designed for APR, it is tested on Defects4J. As reported, CODIT can suggest 16 correct patches. Compared with our results on the benchmark dataset Defects4J, DLFix can find xx patches.

%Hata et al.~\cite{hata2018learning} proposes, Ratchet, a patch
%generation system using the basic attention-based Encoder and Decoder
%machine translation model.
%Similar to Ratchet, Tufano et al.~\cite{tufano2018empirical} use the
%basic encoder-decoder machine translation model and code abstraction
%to generate patches. Furthermore, Tufano et
%al.~\cite{tufano2019learning} propose a deep learning based approach
%for learning code changes using the techniques including code
%abstraction, keywords replacing and neural machine translation
%model. They claim that their approach can be applied to APR. Through
%empirical comparisons, our approach DLFix outperforms them.

%Compared with the above studies using deep learning, our approach is mainly different in the following ways: (1) we develop a new two-layer Tree-based NMT model that is different from any existing NMT model; (2) we do not just learn the context from the changed lines, but also the code surrounding a fix, which makes our model more powerful on learning; and (3) we combine program analysis techniques, such as alpha-renaming and verifying program semantics.


==> demo/fse21-demo-training.tex <==
\subsection{Training Process}

Before explaining the process of code repairing, we first present the
training process for our two-layer, tree-based LSTM model.

\begin{figure}[!htb]
	\centering
	\includegraphics[width=3.4in]{fse21-demo-training-pic}
	\caption{Training for Code Repair}
	\label{fig:training}
\end{figure}

The input for training includes the source code before and after a fix
(Figure~\ref{fig:training}), which are parsed into ASTs. We then use
CPatMiner~\cite{icse19-cpatminer} to compare them to derive the {\em
  changed, inserted}, and {\em removed} subtrees. As a result, the AST
subtrees for the buggy statements are mapped to the respective fixed
subtrees.

Each buggy subtree and its corresponding fixed subtree are used to
training the tree-based LSTM context learning model.
%{\bf 1. Fixing-Context Learning}~(Section~\ref{contextlearning:sec}).
%For each buggy subtree $T$ corresponding to a buggy statement, we need
%to build the fixing context and its corresponding context (step 1). To
%build the fixing context $C_b$ for $T$, we take the AST and collapse
%the structure of $T$ into a summarized node, and replace other buggy
%subtrees in the AST with the corresponding fixed subtrees. The
%corresponding (fixed) context $C_f$ of $T$ is similarly handled as
%$C_b$ with summarization, however, no such replacement is needed
%(because the code is fixed). The pair of $C_b$ and $C_f$ is used for
%training at the input layer and the output layer of a tree-based LSTM
%model~\cite{Tai-2015} (step 2).
The vectors computed from the summarization of buggy subtrees are used
as the additional weights in the code transformation learning model next.
Those additional weights represent the fixing contexts.
%{\bf 2. Code-Transformation Learning}~(Section~\ref{codetrans:sec}).
To learn code transformations for fixing,
%(step 4, Figure~\ref{Fig:train}),
each buggy subtree $T$ itself and its fixed subtree $T'$ after the fix
are used at the input layer and the output layer of another tree-based
LSTM for training.

%Moreover, the fixing context computed as the vector in fixing-context
%learning is used an additional input in this step.

Let us explain in details the two phases in training: 1) training the
tree-based LSTM for {\em context learning}, and 2) training the second
layer of the tree-based LSTM for {\em code transformation learning}.


==> demo/fse21-demo-transformation-learning.tex <==
\subsubsection{Code Transformation Learning}
\label{sec:code-transformation}

\begin{figure}[t]
	\centering
	\includegraphics[width=3.4in]{fse21-demo-transformation-training.png}
	\caption{Code-Transformation Learning}
	\label{Fig:example_trans}
%	\vspace{-4pt}
\end{figure}

We use a LSTM model (same as in Section~\ref{sec:ctx-learning}) to
learn the code transformation for each buggy subtree.
%Let us present how we build the subtrees for the input and output
%layers to train the model from a pair of a buggy $S$-subtree and its
%corresponding fixed $S$-subtree.
Figure~\ref{Fig:example_trans} illustrates the process.
First, for each of the buggy subtrees, the same word embedding process
is applied to produce the corresponding tree structures before and
after the fix. Next, we use the summarized vectors $V_s$ and $V'_s$
computed from fixing-context learning as the weights to perform
cross-product for each node in the buggy subtree and in the fixed
subtree. The two resulting subtrees after cross-product are used at
the input and output layers of the LSTM transformation learning
model. We use cross-product since we aim to have a vector as the
label for a node and use it as a weight representing the context to
learn code transformation.






==> demo/fse21-demo-tree-repair.tex <==
\subsection{Tree-based Code Repair}
\label{treerepair:sec}

\begin{figure}[t]
	\centering
	\includegraphics[width=3.4in]{fse21-demo-tree-fix.png}
%        \vspace{-0.18in}
	\caption{Tree-based Code Repair}
	\label{Fig:repair}
%	\vspace{-0.11in}
\end{figure}

%\begin{figure}[t]
%	\centering
%	\includegraphics[width=3in]{graphs/treepredict}
%	\caption{Tree-based Code Repair}
%	\label{Fig:repair2}
%\end{figure}

After deriving the buggy hunks with one or multiple buggy
statements, we use the trained LSTM models to derive the fixes for
all the buggy hunks at once. Figure~\ref{Fig:repair} illustrates our
process. The AST subtrees for buggy statements are first identified,
e.g., $T1$ and $T2$.

\underline{Step 1.} [Embedding and Summarization] We perform word
    embedding and summarization on all the buggy subtrees. For
    example, we summarize $T1$ into $V_1$ and $T2$ into $V_2$.

\underline{Step 2.} [Predict Context] We use the trained LSTM model
for learning contexts to predict the surrounding context for the
fix. The vectors $V_1$ and $V_2$ become $V'_1$ and $V'_2$ after this
step.

\underline{Step 3.} [Adding Weights] The weights $V_1$ and $V_2$
from Step 1 are used to add to the vectors in the buggy
subtrees $T1$ and $T2$.

\underline{Step 4.} [Predict Transformations] In this step, we use
the trained LSTM model for transformation learning to predict
the subtrees of the fix.

\underline{Step 5.} We remove ``the weight'' from each subtree from
Step 4 to obtain the candidate fixed subtree for each buggy
subtree. For example, we remove the weights $V'_1$ and $V'_2$
to obtain the candidate fixed subtrees.

Because we know the cross product and a vector, we can get the
unlimited number of solutions. Therefore, to produce a single
solution, for each node, we assume that $V'_1$ and $V'_2$ are
vertical with the node vector $V_{n1}$ and $V_{n2}$.
Then, we can get the unweighted node vector $V'_{n1}$ as
follows:
\begin{equation}\label{eq:15}
\begin{split}
V'_{n1} = \frac{V'_1 \times V_{n1}}{V'_1 \dot V'_1}
\end{split}
\end{equation}
After having the vector for each node in a fixed subtree, we generated
candidate patches based on word embedding. For each node, we
calculated the cosine similarity score between its vector $V'_{n1}$
and each vector in the vector list for all tokens. To generate
candidate patches, we select the token $t$ in the list. Token $t$ has
its similarity score $Score_t$ for one node in the fixed subtree. By
adding all $Score_t$ for all the tokens, we have the total score,
$Score_{sum}$, for a candidate. We select the top-5 candidates for
each node to generate the candidates and sort them based on
$Score_{sum}$.

%After deriving the buggy hunk(s) in the method(s), we use
%the trained LSTM models to derive fixes for all the hunks at
%once. For each hunk, we parse the code into AST, and identify the
%buggy $S$-subtrees corresponding to the derived buggy statements.
%In Figure~\ref{Fig:repair}, the $S$-subtrees $T_1$, $T_2$, and $T_3$
%are the buggy $S$-subtrees. If a buggy $S$-subtree is part of another
%larger buggy $S$-subtree, we just need to perform fixing on the
%larger $S$-subtree since that fix also fixes the smaller
%$S$-subtree. In Figure~\ref{Fig:repair}, if we fix the subtree $T_1$
%of the \code{if} statement, that fix includes the fix for the subtree
%$T_3$ ({\em return~a;}).

%First, we perform word embedding and summarization to obtain the
%context. We use GloVe~\cite{glove2014} to produce vectors for all the
%buggy $S$-subtrees to be fixed. We also perform summarization for
%those buggy $S$-subtrees using TreeCaps~\cite{treecaps}.  For example,
%in Figure~\ref{Fig:repair}, $T_1$ and $T_2$ are summarized into two
%vectors $V'_1$ and $V'_2$. Second, the context consisting of the AST
%nodes with the summarized nodes for the buggy $S$-subtrees are used as
%the input for the first trained LSTM model (for context learning) to
%produce the predicted fixing context.  In the AST of the predicted fixing
%context, the structure is the same as the AST for the input context,
%except that the summarized nodes become the new ones. For example,
%$V'_1$ and $V'_2$ in the context becomes $V''_1$ and $V''_2$
%after~prediction.

%Third, we need to compute the weighted buggy $S$-subtrees from the
%buggy $S$-subtrees. To do so, the summarized nodes in the input
%context are used as the additional weights for the respective buggy
%$S$-subtrees. For example, we compute the subtrees $T'_1$ and $T'_2$
%such that each node is represented by a multiplication vector between
%the original vector of the node and the summarized vector $V'_1$ or
%$V'_2$, respectively. Fourth, the weighted buggy $S$-subtrees are used
%as the input for the second trained LSTM model (for code
%transformation prediction) to produce the weighted fixed $S$-subtrees.
%For example, $T'_1$ and $T'_2$ are used as the input to produce
%$T''_1$ and $T''_2$.

%Finally, at step 5, we remove ``the weight'' (i.e., the new summarized
%nodes computed in the predicted context) from each weighted fixed
%$S$-subtree to obtain the candidate fixed $S$-subtree for each buggy
%one. For example, we remove the weights $V''_1$ and $V''_2$ from
%$T''_1$ and $T''_2$ to obtain the candidate fixed $S$-subtrees
%$T_{1f}$ and $T_{2f}$ (not~shown).
%
%For the removal, we perform the following computation.
%Because we know the cross product and a vector, we can get the
%unlimited number of solutions. Therefore, to produce a single
%solution, for each node in $T''_1$ and $T''_2$, we assume that $V''_1$
%and $V''_2$ are vertical with the node vector $V_{n1}$ in $T''_1$ and
%$V_{n2}$ in $T''_2$.
%Then, we can get the unweighted node vector $V'_{n1}$ in $T_{1f}$ as
%follows:
%\begin{equation}\label{eq:15}
%\begin{split}
%V'_{n1} = \frac{V''_1 \times V_{n1}}{V''_1 \dot V''_1}
%\end{split}
%\end{equation}
%After having the vector for each node in a fixed S-subtree $T_{1f}$, we
%generated candidate patches based on word embedding. For each node, we
%calculated the cosine similarity score between its vector $V'_{n1}$
%and each vector in the vector list for all tokens. To generate
%candidate patches, we select the token $t$ in the list. Token $t$ has
%its similarity score $Score_t$ for one node in the fixed
%$S$-subtree. By adding all $Score_t$ for all the tokens, we have the
%total score, $Score_{sum}$, for a candidate. We select the top-5
%candidates for each node to generate the candidates and sort them
%based on $Score_{sum}$.


==> sections/appro.tex <==
\section{Approach}

As we mentioned in approach overview, as for our whole approach, we would like to introduce our work in both training and fixing processes. We would like to introduce each step in following sections.

\input{sections/training}
\input{sections/predicting}


==> sections/buganalysis_2.tex <==
\begin{definition} \label{def:bughunk}
	\textbf{Buggy Hunk: }A chunk of statements that are needed to be fixed in one method.
\end{definition}

For example, in figure \ref{fig:concepts}, within method \textit{example}, the statements at \textit{line 2-5} all are buggy and they all connected together as a chunk. We regard this chunk of buggy statements as a \textbf{buggy hunk}.

\begin{definition} \label{def:hunktype}
	\textbf{Buggy Hunk Types: }There are two types of buggy hunks: one-statement buggy hunk and multi-statements buggy hunk. 
\end{definition}

One-statement buggy hunk is one buggy hunk with only one buggy statement. Multi-statement buggy hunk is one buggy hunk with multiple buggy statements.

As for an example, in figure \ref{fig:concepts}, the buggy hunk includes the statements at \textit{line 2-5} has multiple statements inside. We regard it as a \textbf{multi-statements buggy hunk}.

\begin{definition} \label{def:onebug}
	\textbf{Committed Bug: }One or multiple buggy hunks that are fixed together in one commit are regarded as a \textbf{committed bug}.
\end{definition}

As in figure \ref{fig:concepts}, there is only one buggy hunk that includes the statements at \textit{line 2-5} in one commit, so we regard it as a \textbf{committed bug}.

\begin{definition} \label{def:bugtypes}
	\textbf{Bug Types: }There are four types of committed bugs: bug with one hunk one to one fix, bug with multiple hunks one to one fix, bug with one hunk m to n fix, bug with multiple hunks m to n fix. 
\end{definition}

Bug with one hunk one to one fix is a bug that contains one one-statement buggy hunk. Bug with multiple hunks one to one fix is a bug that contains multiple one-statement buggy hunk. Bug with one hunk m to n fix is a bug that contains one multi-statement buggy hunk. Bug with multiple hunks m to n fix is a bug that contains multiple one-statement buggy or multi-statement buggy hunk, and there is at least one multi-statement buggy hunk.

Within figure \ref{fig:concepts}, there is only one multi-statements buggy hunk that includes \textit{line 2-5} with four statements, so we regard this bug as a \textbf{bug with multiple hunks m to n fix}.

==> sections/bugfixing_2.tex <==
\begin{definition} \label{def:statementsubtree}
	\textbf{Statement Based Sub-tree (SBST): }A sub-tree of AST that exactly represent one statement in the same method without any additional or missing information.
\end{definition}

As for \textit{tree 1} in figure \ref{fig:concepts}, the two nodes that in red box in Buggy Method AST include $return$ and $b$ are connected as a sub-tree. This sub-tree can only represent the statement $return b;$, so we regard it as a \textbf{statement based sub-tree}.

%\begin{definition} \label{def:beforeafter}
	%\textbf{Before Fixing and After Fixing: }Before fixing is the status that the whole AST for the method or the corresponding sub-tree with the bug inside that needs to be automatic fixed. After fixing is the status that the AST or corresponding sub-tree has been fixed.
%\end{definition}

%For example, in figure \ref{fig:concepts}, the \textit{tree 1} is the AST for the method with the bug, so we regarded it as the \textbf{before fixing} AST. In the same way, the \textit{tree 2} is regarded as after fixing AST.

\begin{definition} \label{def:noderepresentation}
	\textbf{AST Node Representation: }A vector generated by GloVe \cite{} that can abstract and represent a AST node.
\end{definition}

To generate vectors to represent AST nodes, we regard each line in source code as a sequence. By using all sequences as input, GloVe generates vectors that can abstract and represent all tokens in source code that are also the AST nodes in AST.

For example, in figrue \ref{fig:concepts}, we use all source code from $buggy method$ and $fixed method$ that contain 13 lines that we regard as 13 sequences as input for GloVe. GloVe generates a list of vector for each token in $buggy method$ and $fixed method$. For example, we can get $V_a$ to represent all nodes $a$ in $buggy method AST$ and $fixed method AST$. Here, $V_a$ is the representation for AST node $a$.


\begin{definition} \label{def:nodefixing}
	\textbf{AST Node Fixing: }A AST node fixing is represented by a triplet of $(<Operation><AST Node><SBST>)$. The $<Operation>$ includes $added$, $deleted$, $modified$.
\end{definition}

We take figure \ref{fig:concepts} as an example. In this figure, the green node $a$ has been changed to $b$ after fixing. If we regard the statement based sub-tree as $subtree_1$. This fix on node $a$ is regarded as $(<modified><a><subtree_1>)$.

\begin{definition} \label{def:subtreefixing}
	\textbf{AST Sub-tree Fixing: }A AST sub-tree fixing is represented by a triplet of $(<SBST><AST Node Fixing List(ANFL)>\\<Statement Level Operation(SLO)>)$. 
\end{definition}

Among the three parameters mentioned above, the $<ANFL>$ is a list of AST node fixings that have the same $<SBST>$ with this AST Sub-tree Fixing. The $<SLO>$ includes $added$, $deleted$, $modified$. If any AST node fixings in $<ANFL>$ with the $modified$ as $<Operation>$, the $<SLO>$ is $modified$. If all $<Operation>$ are $added$, the $<SLO>$ is $added$. If all $<Operation>$ are $deleted$, the $<SLO>$ is $deleted$.

For example, in figure \ref{fig:concepts}, the statement based sub-tree in green box with if statement in buggy method AST has two AST node fixing. The first one is node $>$ has been fixed to $>=$ we regarded as $fix_1$, and the other one is the node $block$ has been added we regarded as $fix_2$. With the situation of this, we regard the $<SLO>$ of this statement based sub-tree is $modified$. If we regard this statement based sub-tree as $subtree_2$. As a summary, the \textbf{AST sub-tree fixing} for this statement based sub-tree is $(<subtree_2><fix_1;fix_2><modified>)$.

\begin{definition} \label{def:subtreesummarize}
	\textbf{Sub-tree Summarization: }A vector generated by tool TreeCaps \cite{} that can be used to abstract and represent an AST sub-tree.
\end{definition}

As we can see in figure \ref{fig:concepts}, we put the $sub-tree 1$ in $buggy method AST$ as input into TreeCaps \cite{}. And the output of TreeCaps is $Vector 1$ that is the \textbf{sub-tree summarization} for $sub-tree 1$.

\begin{definition} \label{def:subtreereplace}
	\textbf{Sub-tree Replacement: }A new AST that all buggy statement based sub-trees that are not under fixing have been replaced by fixed statement based sub-trees.
\end{definition}

We take figure \ref{fig:concepts_2} as an example. In this figure with $buggy method AST$, if the orange node $>$ is under fixing and the $sub-tree 1$ is buggy with the buggy node $a$ and this sub-tree is not under fixing, the sub-tree replacement can come up with the $AST 3$ by replacing $sub-tree 1$ with the $sub-tree 2$ from $fixed method AST$ that is the fixed version of $sub-tree 1$.

%\begin{definition} \label{def:vectorrepresentation}
	%\textbf{Representation Vector: }A vector generated by a learning tool from text that can abstract and represent a piece of code, an AST node or an AST sub-tree.
%\end{definition}

%To show the detail, we could use figure \ref{fig:concepts} as an example. In figure \ref{fig:concepts}, $V_a$ is a \textbf{representation vector} learned by word2vec \cite{}, and $V_a$ can represent the green node $a$ in $Tree 1$.


%\begin{definition} \label{def:summarizednode}
	%\textbf{Summarized Vector: }A representation vector that can abstract and represent a corresponding sub-tree.
%\end{definition}

%As in figure \ref{fig:concepts}, $V_{green}$ is a representation vector learned by TreeCaps \cite{}, and $V_{green}$ can represent the green sub-tree in $Tree 1$. We regard $V_{green}$ as a \textbf{summarized vector}.




==> sections/conce.tex <==
\section{Main Concepts}

%\begin{figure*}[h]
%	\centering
%	\includegraphics[scale=0.14]{graphs/figure_1.png}
%	\caption{Testing Process of Our Approach}
%	\label{Fig:concepts}
%\end{figure*}

%Let us present the main concepts used in our work.

%In this section, before we talking about our approach, we would like to introduce some important concepts that we need to use in the following sections. We talk about these concepts in two direction: \textit{bug analysis} and \textit{bug fixing}.

\subsection{Fix Representation}

{\tool} uses AST as a representation for source code because it
captures the syntactical structure before and after a
fix. Figure~\ref{Fig:diff} shows an example of the ASTs of the code
before and after a fix. We use CPatMiner~\cite{icse19-cpatminer} to
derive structural changes for a fix.

\begin{Definition}[{\bf Fixing Change}]
A (fine-grained) fixing change is represented by a triplet of
{\bf \code{(<operation kind>, <AST node type>, <label>)}}.
\end{Definition}

Each fixing change corresponds to {\em a change to an AST~node} in the
program.  We consider each change to be one of the following
operations: \code{update}, \code{insert}, and \code{delete}. The AST
node types represent the Java AST nodes and labels represent 
their textual information.

%of the AST nodes.

\begin{figure}[t]
	\centering
	\includegraphics[width=5in]{graphs/diff_new2.png}
        %\vspace{-0.20in}
	\caption{ASTs before and after a fix}
       % \vspace{-0.04in}
	\label{Fig:diff}
\end{figure}

In Figure~\ref{Fig:diff}, the \code{Return Stmt} node for the \code{else}
branch is an \code{insert} one. The corresponding fixing change is
\code{($<$insert$>$}, \code{$<$return$>$}, \code{`return true;'}). The
assignment \code{$a =a + 1;$} was \code{updated} into \code{$a =a -
  b;$} because its subtree contains the nodes that were updated,
inserted, or deleted. In this case, we consider \code{$a =a + 1;$} as
a changed/fixed statement. The \code{Val} node for the value 1 in the
AST before the fix is considered as \code{deleted}, while the
\code{Var} node for the variable \code{b} after the fix is \code{inserted}.

\begin{Definition}[{\bf Buggy Statement Subtree ($S$-subtree)}]
A buggy subtree is a subtree that is labelled as \code{update} or
\code{delete}. If such as subtree corresponds to a statement, it is
called buggy statement subtree.
%~($S$-subtree).
\end{Definition}

An example of a buggy $S$-subtree is the subtree \code{ASGN}
corresponding to the statement at line 5 of Figure~\ref{fig:motiv},
because it was \code{updated}.

%In Figure~\ref{Fig:diff}, $T$ is considered a buggy $S$-subtree.

%Each buggy $S$-subtree has a corresponding {\em fixed $S$-subtree},
%which is identified by the AST-based differencing tool. For example,
%$T'$ is the fixed $S$-subtree of $T$. In the case of deletion, the
%corresponding subtree is an {\em empty} tree. For an inserted
%statement $S\_ins$, we handle the parent statement of $S\_ins$ as it is
%marked as an \code{updated} statement.

\begin{Definition}[{\bf Summarized Node and Summarized Vector}]
  A summarized node is used to replace a buggy $S$-subtree in the AST
  and is represented by a summarized vector, which is computed via an
  encoding method to capture the structure of the $S$-subtree.
\end{Definition}

%In the example, the \code{IF} node $T$ is ``summarized''
%into a summarized node $S_T$ (not shown).
In {\tool}, we use GloVe~\cite{glove2014} learning representation to
encode an AST subtree, which has been shown to have the capability to
capture well the code structure. Any other code learning
representation method could be used.
%
In a fix involving multiple statements, there are multiple buggy
$S$-subtrees. Thus, we could have multiple summarized nodes. In
Figure~\ref{fig:motiv}, we have two summarized nodes for the two
$S$-subtrees for the statements at line 5 and line 10.

\begin{Definition}[{\bf Fixing Context}]
  The fixing context of a buggy $S$-subtree is the AST of the entire method in
  which the $S$-subtree is replaced with its summarized node and for
  any other buggy $S$-subtree, we replace it with the respective fixed
  subtree in the AST after the fix.
\end{Definition}

In Figure~\ref{fig:motiv}, the fixing context of the $S$-subtree
of the statement at line 5 (\code{retrieved\_password} =
\code{getPassword(UID);} is the entire AST of the method
in which that $S$-subtree is replaced with a summarized node and
the $S$-subtree corresponding to the statement at line 10:

\code{boolean password\_check = compare(password, retrieved\_password);}

is replaced with the fixed subtree of the fixed code:

\code{boolean password\_check = compare(passwordHash(password),retrieved\_password);}

%The idea is that we would like to provide the correct code context for
%a model to learn the proper fix as explained earlier.

We will explain the embedding representations for AST subtrees and
nodes to be used in the LSTM models later.

%Finally, we encode the buggy $S$-subtrees, the corresponding fixed subtrees,
%and the summarized nodes, and the fixing contexts by vector representations
%to be used in deep learning models. We will explain such encoding later.

\subsection{Bug Types}\label{types}

\begin{Definition}[{\bf Buggy Hunk}]
A buggy hunk is a code fragment containing one or multiple
  consecutive buggy statements in a method.
\end{Definition}

Figure~\ref{fig:motiv} contains a buggy hunk with the buggy statements
at line 5 and line 10, which are consecutive in the original buggy code.

In general, to fix a bug, one could make changes involving one
or multiple buggy hunks. For each hunk, one or multiple buggy statements
might be changed. Thus, we have the following types:

\begin{Definition}[{\bf Bug Types}]
We have the following bug types:
  
{\em \bf Type-1. One Hunk One-Statement}: A bug with the fix involving only one hunk and one statement in the hunk.

{\em \bf Type-2. One Hunk Multi-Statements}: A bug with the fix involving only one hunk and multiple statements in that hunk.

{\em \bf Type-3. Multi-Hunks One-Statement}: A bug with the fix involving multiple hunks and each hunk having one fixed statement.

{\em \bf Type-4. Multi-Hunks Multi-Statements}: A bug with the fix involving multiple hunks and each hunk having multiple statements.

{\em \bf Type-5. Multi-Hunks Mix-Statements}: A bug with the fix involving multiple hunks and some hunks
having one statement and some others having multiple ones.

\end{Definition}

%==========================
%As for \textit{bug analysis}, before we do the fixing, we analysis the bugs to clarify the challenge of our fixing problem. The following concepts are about bug types:

%\input{sections/buganalysis}

%As for \textit{bug fixing}, because the Abstract Syntax Tree (AST) can represent the information for both the meaning of the code and the structure of the code, when doing the bug fixing, we would like to use AST to analysis and do the fixing. The following concepts are related to AST: 

%\input{sections/bugfixing}




%\begin{definition} \label{def1}
	%\textbf{Node Change Detection: }
	
	%\textbf{Node Change Detection: } A node level AST-based tree differencing analysis to figure out what nodes have been modified, added, or deleted between the buggy version and the fixed version of the code.
%\end{definition}

%\begin{definition} \label{def2}
	%\textbf{Direct Data Dependency: } A direct linkage (one step distance) during the data flow analysis for two statements.
%\end{definition}

%\begin{definition} \label{def3}
	%\textbf{AST-based Change Detection: } A statement mapping detection from the buggy version of the code to the fixed version of the code based on the node change detection results (definition \ref{def1}) and direct data dependency (definition \ref{def2}).
%\end{definition}

%\begin{definition} \label{def4}
	%\textbf{AST Sub-tree: } A sub-tree structure from AST that all nodes in it could be fully covered by one or multiple statements and all tokens in these one or multiple statements could also be fully covered by the sub-tree structure at the same time.
%\end{definition}

%\begin{definition} \label{def5}
	%\textbf{Sub-tree Summarization: } A process of getting a summarized vector that be used to abstract and represent a AST sub-tree (definition \ref{def4}) and replacing the AST sub-tree with the summarized vector.
%\end{definition}

%\begin{definition} \label{def6}
	%\textbf{Sub-tree Replacing: } A process of replacing the buggy version of a AST sub-tree (definition \ref{def4}) with the fixed version of it.
%\end{definition}

%\begin{definition} \label{def7}
%	\textbf{Buggy Hunk: } A set of buggy statements that one statement follows one statement in the source code are collected as a \textbf{buggy hunk}.
%\end{definition}

%\begin{definition} \label{def8}
	%\textbf{Context Fixing: } A process of generating a fixed summarized vector for a buggy statement with the context information of the surrounding statements.
%\end{definition}

%\begin{definition} \label{def9}
%	\textbf{Code Transformation: } A group of changes in the same buggy hunk (definition \ref{def7}) from the buggy version of the code to the fixed version of the code.
%\end{definition}

%\begin{definition} \label{def10}
%	\textbf{Multi-Statements Expansion: } A process of increasing the buggy statement number in a buggy hunk (definition \ref{def7}) based on the direct data dependency (definition \ref{def2}) and a buggy statement classifier.
%\end{definition}

%\begin{definition} \label{def11}
%	\textbf{Buggy Statement Grouping: } A process of grouping the buggy statements in the same buggy hunk (definition \ref{def7}) into different groups based on the AST-based change detection results (definition \ref{def3}) and the node change detection results (definition \ref{def1}).
%\end{definition}


==> sections/conce_2.tex <==
\section{Definition}

\begin{figure*}[h]
	\centering
	\includegraphics[scale=0.29]{graphs/figure_3.png}
	\caption{Example 1 for Concepts}
	\label{fig:concepts}
\end{figure*}

In this section, before we talking about our approach, we would like to introduce some important concepts that we need to use in the following sections. We talk about these concepts in two direction: \textit{bug analysis} and \textit{bug fixing}.

As for \textit{bug analysis}, before we do the fixing, we analysis the bugs to clarify the challenge of our fixing problem. The following concepts are about bug types:

\input{sections/buganalysis_2}

\begin{figure}[h]
	\centering
	\includegraphics[scale=0.20]{graphs/figure_2.png}
	\caption{Example 2 for Concepts}
	\label{fig:concepts_2}
\end{figure}

As for \textit{bug fixing}, because the Abstract Syntax Tree (AST) can represent the information for both the meaning of the code and the structure of the code, when doing the bug fixing, we would like to use AST to analysis and do the fixing. The following concepts are related to AST: 

\input{sections/bugfixing_2}




%\begin{definition} \label{def1}
	%\textbf{Node Change Detection: }
	
	%\textbf{Node Change Detection: } A node level AST-based tree differencing analysis to figure out what nodes have been modified, added, or deleted between the buggy version and the fixed version of the code.
%\end{definition}

%\begin{definition} \label{def2}
	%\textbf{Direct Data Dependency: } A direct linkage (one step distance) during the data flow analysis for two statements.
%\end{definition}

%\begin{definition} \label{def3}
	%\textbf{AST-based Change Detection: } A statement mapping detection from the buggy version of the code to the fixed version of the code based on the node change detection results (definition \ref{def1}) and direct data dependency (definition \ref{def2}).
%\end{definition}

%\begin{definition} \label{def4}
	%\textbf{AST Sub-tree: } A sub-tree structure from AST that all nodes in it could be fully covered by one or multiple statements and all tokens in these one or multiple statements could also be fully covered by the sub-tree structure at the same time.
%\end{definition}

%\begin{definition} \label{def5}
	%\textbf{Sub-tree Summarization: } A process of getting a summarized vector that be used to abstract and represent a AST sub-tree (definition \ref{def4}) and replacing the AST sub-tree with the summarized vector.
%\end{definition}

%\begin{definition} \label{def6}
	%\textbf{Sub-tree Replacing: } A process of replacing the buggy version of a AST sub-tree (definition \ref{def4}) with the fixed version of it.
%\end{definition}

%\begin{definition} \label{def7}
%	\textbf{Buggy Hunk: } A set of buggy statements that one statement follows one statement in the source code are collected as a \textbf{buggy hunk}.
%\end{definition}

%\begin{definition} \label{def8}
	%\textbf{Context Fixing: } A process of generating a fixed summarized vector for a buggy statement with the context information of the surrounding statements.
%\end{definition}

%\begin{definition} \label{def9}
%	\textbf{Code Transformation: } A group of changes in the same buggy hunk (definition \ref{def7}) from the buggy version of the code to the fixed version of the code.
%\end{definition}

%\begin{definition} \label{def10}
%	\textbf{Multi-Statements Expansion: } A process of increasing the buggy statement number in a buggy hunk (definition \ref{def7}) based on the direct data dependency (definition \ref{def2}) and a buggy statement classifier.
%\end{definition}

%\begin{definition} \label{def11}
%	\textbf{Buggy Statement Grouping: } A process of grouping the buggy statements in the same buggy hunk (definition \ref{def7}) into different groups based on the AST-based change detection results (definition \ref{def3}) and the node change detection results (definition \ref{def1}).
%\end{definition}

==> sections/contextoutput.tex <==
\subsubsection{Building Corresponding Context for Output Layer}

%Similar as input layer, we built the corresponding context for the output layer. We used corresponding fixed S-subtree $T_f$ and corresponding AST $AST_f$ for the fixed version of method that contains the fixed buggy sub-tree $T_f$ to prepare the output layer.

%add example here
%To get the summarization vector, we did the same as input layer by using fixed S-subtree $T_f$ as input and got $v_f$ as output from TreeCaps. And then we replaced fixed S-subtree $T_f$ on the AST of the fixed version method $AST_f$ with summarized vector $v_f$ as a AST node.
%add example here
%As for the fixing context building, with the reason for doing S-subtree replacing we mentioned in input layer building, for each fixed S-subtree $T_f$, because all buggy S-subtrees has already been saved, there is no need for us to do the replacing here. After this step, we had fixing context $AST'_f$ for corresponding fixed S-subtree $T_f$.
%add example here
%We also did in the same way to encode the fixing context $AST'_f$ into encoded fixing context $AST^{encoded}_f$. We had it as the training target for the decoder when doing the training. What's more, we also saved the summarized vector $v_f$ as a weight for the next step usage.

Similar as input layer, we built the corresponding context for the output layer. We did the encoding for Fixed AST $AST_f$. In figure \ref{Fig:example_context}, the \textit{(2) Fixed AST} has been encoded by GloVe into \textit{(4)Encoded Fixed AST}. And then we did the node summarization. We got $V_f$ instead $V_b$ for the fixed S-subtree $T_f$ which just the almost the same as \textit{(5) AST with Summarized Node} in figure \ref{Fig:example_context}. Just used $V_f$ instead of $V_b$ in it. And next, we did the corresponding context building. It is a little bit different from input layer. For example, as you can see in figure \ref{Fig:example_context}, the S-subtree in red box in \textit{(4) Encoded Fixed AST} is already in the fixed version. So there is no need to do the S-subtree replacing as we did in input layer. With the steps of these, we got the fixing context $AST'_f$ for fixed S-subtree $T_f$ which is the training target for the decoder when doing the training. What's more, we also saved the summarized vector $V_f$ we got in this layer as a weight for the next step usage.

==> sections/faultlocalization.tex <==
\subsection{Fault Localization with Buggy Hunks Detection}

%When here comes a new bug, in order to do the automatic fixing, 
%we used existing spectrum based fault localization Ochiai~\cite{abreu2006evaluation} 
%to get the fixing positions. 

Given a program, we apply a fault localization technique to localize a list of suspicious statements that require a fix. Conceptually, 


We used the whole java project as input and the Ochiai provided a list of possible possible fault locations $L_b$ sorted by the scores. 
Because in real bugs, there are many bugs need to fix multiple positions, we identified siblings which are similar possible fixing positions for each fault location in the $L_b$ based on the relevance of fault locations and version history analysis. 
This idea has been proved to be useful in finding multi-hunk bugs in recent study \cite{hercules-icse19}. 
Here we used a fault location in $L_b$ as input to find the siblings and we got the buggy statements locations as output. We used these buggy statement locations in next step.




==> sections/reranking.tex <==
\subsection{Result Candidates Re-ranking}

In this step, we would like to train a re-ranking model to re-rank all possible fixing candidates we got from code transformation learning section 
